Time-Space Tradeoffs for Element Distinctness and Set Intersection via Pseudorandomness

In the Element Distinctness problem, one is given an array $a_1,\dots, a_n$ of integers from $[poly(n)]$ and is tasked to decide if $\{a_i\}$ are mutually distinct. Beame, Clifford and Machmouchi (FOCS 2013) gave a low-space algorithm for this problem running in space $S(n)$ and time $T(n)$ where $T(n) \le \widetilde{O}(n^{3/2}/S(n)^{1/2})$, assuming a random oracle (i.e., random access to polynomially many random bits). A recent breakthrough by Chen, Jin, Williams and Wu (SODA 2022) showed how to remove the random oracle assumption in the regime $S(n) = polylog(n)$ and $T(n) = \widetilde{O}(n^{3/2})$. They designed the first truly $polylog(n)$-space, $\widetilde{O}(n^{3/2})$-time algorithm by constructing a small family of hash functions $\mathcal{H} \subseteq \{h | h:[poly(n)]\to [n]\}$ with a certain pseudorandom property. In this paper, we give a significantly simplified analysis of the pseudorandom hash family by Chen et al. Our analysis clearly identifies the key pseudorandom property required to fool the BCM algorithm, allowing us to explore the full potential of this construction. As our main result, we show a time-space tradeoff for Element Distinctness without random oracle. Namely, for every $S(n),T(n)$ such that $T\approx \widetilde{O}(n^{3/2}/S(n)^{1/2})$, our algorithm can solve the problem in space $S(n)$ and time $T(n)$. Our algorithm also works for a related problem Set Intersection, for which this tradeoff is tight due to a matching lower bound by Dinur (Eurocrypt 2020). As two additional contributions, we show a more general pseudorandom property of the hash family, and slightly improve the seed length to sample the pseudorandom hash function.

==> backup.tex <==

\subsection{The Recursive Perspective of the Walk}

The walk on the graph $G_{H, a}$ has a natural tree structure: starting with a vertex $x\in [n]$ and $y = a_x\in [m]$, the walk will first move according to $h_{<t}$ for (roughly) $2^{t-1}$ steps until reaching a point $y\in [m]$ where $h_{<t}(y) \equiv 0$. Then the walk makes a level-$t$ move $y\mapsto a_{h_t(y)}$ and proceeds to a new segment of lower level moves. To better exploit the tree structure, we consider a recursion-based perspective of the walk on the graph $G_{H, a}$, as shown in Algorithm~\ref{algo:standard-walk}. Algorithm~\ref{algo:standard-walk} starts with a given input $x\in [n]$ and produces a (infinite size) tensor $T\colon \mathbb{N}^t \to [n]\cup \{\star\}$. In the following, we also use $\walk^{\std}$ to refer to Algorithm~\ref{algo:standard-walk} and use $T=\walk^\std(h, x)$ to denote the result tensor when running $\walk^\std$ on $h$ with start vertex $x$.

\begin{algorithm2e}[H]
\caption{The Standard Walk}
\label{algo:standard-walk}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwVariable}{Global Variables}              % set the Output
\LinesNumbered

\DontPrintSemicolon
  
    \KwInput{$n,m\ge 1$. $t$ hash functions $h_1,\dots, h_t$. The input array $a_1,\dots, a_n$. The start vertex $x\in [n]$.}
    
    % Set Function Names
    \SetKwFunction{FMain}{Main}
    \SetKwFunction{FWalk}{walk}
    \SetKw{Break}{break}
    
    \KwVariable{
        \; ~~~~ A tensor $T:\mathbb{N}^t\to [n]\cup \{\star\}$. Initialized with $\star$'s.
    }
    
    \SetKwProg{Fn}{Program}{:}{\KwRet}
    \Fn{\FMain}{
        $\ell \gets (0, 0, \dots, 0) \in \mathbb{N}^{t}$ \;
        $T(\ell) \gets x$ \;
        $x \gets a_x$ \;
        walk($t$, $x$, $\ell$) \;
        \KwRet $T$\;
    }
    
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FWalk{$i$, $x$, $\ell$}}{
        \If{$i=0$}{
            \KwRet $x$ \;
        }
        \While{\emph{True}}{
            $x\gets $ walk($i-1$, $x$, $\ell$) \;
            $\ell_i \gets \ell_i + 1$ \;
            \If{$h_i(x) = 0$}{
                \Break ;
            }
            \Else{
                $T(\ell) \gets h_i(x)$ \;
                $x\gets a_{h_i(x)}$ \;
            }
        }
        \KwRet $x$\;
    }
\end{algorithm2e}

\begin{remark}
Note that Algorithm~\ref{algo:standard-walk} will eventually visit the same vertex $x\in [m]$ twice and enter a loop. Hence, Algorithm~\ref{algo:standard-walk} cannot really reach Line $6$ in its execution. We include Line $6$ in the pseudo-code only for better exhibition. Nevertheless, the vector $\ell$ in $\walk(*, *, \ell)$ is always getting larger, and the algorithm never updates the same entry $T(\ell)$ twice. Therefore, the tensor $T$ is always well-defined.
\end{remark}

\subsubsection{Understanding the standard walk}

Before we continue, we set up necessary pieces of notation and state some basic facts about the structure of $\walk^\std$. We start with the definition of ``index'' to the tensor $T$.

\begin{definition}\label{def:index}
We use the term \emph{index} to refer to $t$-dimensional integer vectors $\ell = (\ell_1,\dots, \ell_t)$. Given an index $\ell$, we use $T(\ell)$ to denote the $\ell$-th entry of $T$. We introduce the following total ordering for indices: for two indices $\ell^1 \ne \ell^2$, let $i\in [t]$ be the \emph{largest} integer such that $\ell^1_i \ne \ell^2_i$. Then we say $\ell^1 < \ell^2$ if $\ell^1_i < \ell^2_i$. The width of an index $\ell$ is defined as $\width(\ell) := \max_{1\le i\le t} \{ \ell_i \}$. We call an index $\ell$ $\tau$-bounded if $\width(\ell) \le \tau$. We define the level of an index as $\level(\ell) := \max\{q : \forall i< q, \ell_i = 0\}$. In particular, we define $\level(\vec{0}) := t + 1$. For every $0\le i\le t$, we use $\ell_{<i}, \ell_{>i}$ to denote the length-$i$ prefix and length-$(t-i)$ suffix of $\ell$, respectively.
\end{definition}

Throughout the whole article, we reserve the letter ``$\ell$'' and ``$r$'' for indices to tensors. 

When Line TODO - TODO is executed in a function call $\walk(i, x, \ell)$, we say the algorithm makes a level-$i$ move. Note that we use the index $\ell$ in the function call to track the ``progress'' of the walk. The index should be interpreted as follows. Suppose we call $\walk(i, x, \ell)$ with $\ell = (\ell_1, \ell_2,\dots, \ell_t)$. Then it is always guaranteed that $\level(\ell) > i$. For the part $\ell_{>i}$, $\ell_{t}$ counts the number of level-$t$ moves before reaching $\walk(i, x, \ell)$. For every $j\in [i+1, t-1]$, $\ell_{j}$ further counts the number of level-$j$ moves after the very last level-$(j+1)$ move. 

\subsubsection{Analyzing the standard walk} 

Back to our discussion, we first observe that the tensor $T$ exactly represents the set $\Out_{a,H}(x)$ in the sense that
\[
\Out_{a,H}(x) = \{ u\in [n]: \exists \ell\in \mathbb{N}^t, T(\ell) = u \}.
\]
Now, consider sampling a list of random $\mathbf{h}_1,\dots, \mathbf{h}_t$ together with a start vertex $\mathbf{x}$. Let $\mathbf{H}, \mathbf{T}$ be two random variables denoting the result hash function and tensor, respectively. We wish to find the probability that $u,v\in \Out_{a,\mathbf{H}}(\mathbf{x})$. By the observation above, we can translate this probability to a probability regarding $\mathbf{T}$ as follows.
\begin{align}
& ~~~~ \Pr_{\mathbf{h_1},\dots, \mathbf{h}_t, \mathbf{x}}[u,v\in \Out_{a,\mathbf{H}}(\mathbf{x})] 
 \notag \\ 
 & = \sum_{\ell^1 < \ell^2}\Pr_{\mathbf{h}_1,\dots,\mathbf{h}_t, \mathbf{x}}\left[  \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \left( \forall \ell^3 < \ell^4 < \ell^2, \mathbf{T}(\ell^3) \not\simeq \mathbf{T}(\ell^4) \right)\right]. \label{eq:translate-to-tree}
\end{align}
Set a threshold $\tau = 5\log n$. Next, our goal is to lower bound for each \emph{$\tau$-bounded} (see Definition~\ref{def:index}) pair $(\ell_1, \ell_2)$ the probability in \eqref{eq:translate-to-tree} by $c\cdot \frac{2^{-|\ell_1|-|\ell_2|}}{n^2}$ for some constant $c > 0$. Assuming this is true for now, we can easily deduce that
\begin{align}
& \sum_{\ell^1 < \ell^2: \text{both $\tau$-bounded} }\Pr_{\mathbf{h}_1,\dots,\mathbf{h}_t, \mathbf{x}}\left[  \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \left( \forall \ell^3 < \ell^4 < \ell^2, \mathbf{T}(\ell^3) \not\simeq \mathbf{T}(\ell^4) \right)\right] \notag \\
& \ge \frac{1}{2} \left( \sum_{\ell^1, \ell^2: \text{both  $\tau$-bounded}} \frac{c\cdot 2^{-|\ell_1|-|\ell_2|}}{n^2} - \sum_{\ell^1 = \ell^2: \text{$\tau$-bounded}} \frac{c\cdot 2^{-2|\ell^1|}}{n^2}  \right) \notag \\ 
& \ge \frac{c}{2\cdot n^2} \left( \sum_{i=0}^{\tau-1} 2^{-i} \right)^{2t} - \frac{c}{n^2} \left( \sum_{i=0}^{\tau-1} 2^{-2i} \right)^t \notag \\
& \ge \Omega\left(\frac{2^{2t}}{n^2}\right) - O\left(\frac{2^t}{n^2}\right) \ge \Omega\left( \frac{1}{n} \right). \label{eq:main-lowerbound}
\end{align}
In the following, we introduce new tools (``extended walks'') to prove the lower bound for each and every $\tau$-bounded pair $(\ell^1,\ell^2)$.

\subsection{The Extended Walk}
 
Analyzing the distribution $(\mathbf{T}(\ell^1), \mathbf{T}(\ell^2))$ through $\walk^\std$ directly seems very hard. To circumvent the issue, we will couple the standard walk with a family of carefully designed extended walks. For any finite set $S\subseteq \mathbb{N}^t$ of indices, we construct an $S$-extended walk as shown in Algorithm~\ref{algo:extended-walk}. In the following, we also use $\walk^S$ to denote the $S$-extended walk and use $\mathbf{T}^S \sim \walk^S(h,x)$ to denote the tensor\footnote{Note that even if $h, x$ are fixed, the extended walk still has its internal randomness.} produced by running $\walk^S$ on $h$ with start vertex $x$. 
%We use $\supp(\walk^S(h,x))$ to denote the support of $\walk^S(h,a)$.

\begin{algorithm2e}[H]
\caption{The $S$-Extended Walk}
\label{algo:extended-walk}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwVariable}{Global Variables}              % set the Output
\LinesNumbered
\DontPrintSemicolon
  
    \KwInput{
        \; ~~~~ $n,m, t\ge 1$. $t$ hash functions $h_1,\dots, h_t$. The input array $a_1,\dots, a_n$.
        \; ~~~~ A start vertex $x\in [n]$. 
        \; ~~~~ A set of indices $S \subseteq \mathbb{N}^t$.
    }
    
    % Set Function Names
    \SetKwFunction{FMain}{Main}
    \SetKwFunction{FWalk}{walk}
    \SetKw{Break}{break}
    
    \KwVariable{
        \; ~~~~ A constant $\tau \gets 5 \log n$
        \; ~~~~ A tensor $T:[\tau]^t\to [n]\cup \{\star\}$, initialized with $\star$'s
        \; ~~~~ $t$ sets $D_1,D_2,\dots, D_t$, each initialized with $\emptyset$
    }
    
    \SetKwProg{Fn}{Program}{:}{\KwRet}
    \Fn{\FMain}{
        $\ell \gets (0, 0, \dots, 0) \in \mathbb{N}^{t}$ \;
        $T(\ell) \gets x$ \;
        $x \gets a_x$ \;
        walk($t$, $x$, $\ell$) \;
        \KwRet $T$\;
    }
    
    % Write Function with word ``Function''
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FWalk{$i$, $x$, $\ell$}}{
        \If{$i=0$}{
            \KwRet $x$ \;
        }
        \While{$\ell_i < \tau$}{
            $x\gets $ walk($i-1$, x, $\ell$) \;
            $\ell_i \gets \ell_i + 1$ \;
            \If{$\ell \in P(S)$ and $x\in D_i$}{
                Sample $(a,b)\gets_R \{0,1\}\times [n]$ \;
            }
            \Else{
                \If{$h_i(x) = 0$}{
                    $(a,b)\gets (0, 0)$ \;
                }
                \Else{
                    $(a,b)\gets (1, h_i(x))$ \;
                }
            }
            \If{$a = 0$}{
                \Break \;
            }
            \Else{
                \If{$\ell \in P(S)$}{
                    $D_i \gets D_i \cup \{x\}$ \;
                }
                $T(\ell) \gets b$ \;
                $x\gets a_b$ \;
            }
        }
        \KwRet $x$\;
    }   
\end{algorithm2e}


Compared with $\walk^\std$, we implement two major modifications in $\walk^S$:
\begin{itemize}
    \item First, we set a threshold $\tau = 5 \log n$, and require that inside each function call $\mathrm{walk}(i, x, \ell)$, the algorithm makes at most $\tau$ steps of level-$i$ move (See Line $10$). This ensures that the algorithm always has a chance of visiting $\ell^2$ (Otherwise, the walk could enter a loop earlier and never reach $\ell^2$).
    \item Second, we use $t$ sets $D_1, \dots, D_t \subseteq [n]$ to ``remember'' the coordinates of $h_1,\dots, h_t$ that we have probed along $P(S)$ (Line $23$-$24$). When moving along $P(S)$ and trying to access $h_i(x)$, we always check if $h_i(x)$ has been used for previous indices of $P(S)$ (Line $13$). If so, we sample a uniform one-time edge to replace $h_i(x)$ (Line $14$).
\end{itemize}

\subsection{Analyzing the extended walk}

The extended walk behaves nicely if we are only interested in $\mathbf{T}^S(\ell)$ for those $\ell\in S$. Formally, we have the following lemma.

\begin{lemma}\label{lemma:extend-is-random}
Let $S = \{ \ell^1, \dots, \ell^k \}$. Suppose $\mathbf{h}_1,\dots, \mathbf{h}_t$ are $k\tau$-wise independent and the start vertex $\mathbf{x}\sim [n]$ is uniformly chosen. Let $\mathbf{T}^S\sim \walk^S(\mathbf{h}, \mathbf{x})$. For every $u_1,u_2,\dots, u_k \in [n]$, we have
\[
\Pr_{\mathbf{h}, \mathbf{x}, \mathbf{T}^S} \left[ \mathbf{T}^S(\ell^i) = u_i, \forall i\in [1,k] \right] = \frac{2^{-|P(S)|+1}}{n^{k}}.
\]
\end{lemma}

Second, we have the following.

\begin{lemma}\label{lemma:extend-lb-standard}
For every list of hashes $h_1,\dots, h_t$ and start vertex $x\in [n]$, consider the standard walk $T = \walk^{\std}(h, x)$. For every set $S= \{ \ell^1 < \ell^2 < \dots < \ell^k\}$ of $\tau$-bounded indices and every $u_1,\dots, u_k\in [n]$, it holds that
\[
\begin{aligned}
&~~~~ \mathbbm{1} \left\{ \left(  T(\ell^i) = u_i, \forall i\in [k] \right) \land \left( \forall r^1 < r^2<  \ell^k, T(r^1)\not\simeq T(r^2)\right)\right\} \\
&\ge \Pr_{\mathbf{T}^S\sim \walk^S(h, a)} \left[ \mathbf{T}^S(\ell^i) = u_i, \forall i\in [k] \right] -\\
&~~~~ \sum_{\substack{r^1 < r^2 < \ell^k \\ A = \{r^1, r^2\}}} \Pr_{\mathbf{T}^{S\cup A} \sim \walk^{S\cup A}(h, a)} \left[ \left(  \mathbf{T}^{S\cup A}(\ell^i) = u_i, \forall i\in [k] \right) \land (\mathbf{T}^{S\cup A}(r^1) \simeq \mathbf{T}^{S\cup A}(r^2)) \right] - \\
&~~~~ \sum_{\substack{r^3 < \ell^k \\ A = \{r^3\}} } \Pr_{\mathbf{T}^{S\cup A} \sim \walk^{S\cup A}(h, a)} \left[ \left(  \mathbf{T}^{S\cup A}(\ell^i) = u_i, \forall i\in [k] \right) \land \mathbf{T}^{S\cup A}(r^3)\ne \star \right].
\end{aligned}
\]
\end{lemma}

Lemma~\ref{lemma:extend-lb-standard} is somewhat remarkable in that it holds for every fixed $h$ and $x$. One can naturally extend Lemma~\ref{lemma:extend-lb-standard} to an average version by taking expectations over $\mathbf{h}$ and $\mathbf{x}$ (We will use the average version in all applications).

\subsection{Wrapping-up}

Finally, we are ready to conclude the proof. Let us first recall \eqref{eq:translate-to-tree}, re-stated below.
\begin{align}
& ~~~~ \Pr_{\mathbf{h_1},\dots, \mathbf{h}_t, \mathbf{x}}[u,v\in \Out_{a,\mathbf{H}}(\mathbf{x})] 
 \notag \\ 
 & = \sum_{\ell^1 < \ell^2}  \Pr_{\mathbf{h}_1,\dots,\mathbf{h}_t, \mathbf{x}}\left[  \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \left( \forall \ell^3 < \ell^4 < \ell^2, \mathbf{T}(\ell^3) \not\simeq \mathbf{T}(\ell^4) \right)\right]. \label{eq:translate-to-tree-2}
\end{align}

Recall the threshold $\tau = 5\log n$. We only consider the contribution from $\tau$-bounded pairs to the right hand side of \eqref{eq:translate-to-tree-2}. Fix one such pair $(\ell^1, \ell^2)$. By Lemma~\ref{lemma:extend-is-random} and \ref{lemma:extend-lb-standard}, we have:
\[
\begin{aligned}
& ~~~~ \Pr_{\mathbf{h}_1,\dots,\mathbf{h}_t, \mathbf{x}}\left[  \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \left( \forall \ell^3 < \ell^4 < \ell^2, \mathbf{T}(\ell^3) \not\simeq \mathbf{T}(\ell^4) \right)\right]  \\
& \ge \Pr_{\mathbf{T} \sim \mathbf{T}^{\{\ell^1,\ell^2\}}}[ \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} ] - \\
& ~~~~ \sum_{\ell^3 < \ell^4 < \ell^2} \Pr_{\mathbf{T} \sim \mathbf{T}^{\{\ell^1,\ell^2, \ell^3, \ell^4\}}}[ \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \mathbf{T}(\ell^3) \simeq \mathbf{T}(\ell^4) ] - \\
& ~~~~ \sum_{\ell^5 < \ell^2: \width(\ell^5) = \tau} \Pr_{\mathbf{T} \sim \mathbf{T}^{\{\ell^1,\ell^2,  \ell^5\}}}[ \{ \mathbf{T}(\ell^1), \mathbf{T}(\ell^2)\} = \{u, v\} \land \mathbf{T}(\ell^5) \ne \star ] \\
& \ge \frac{2^{1-|P(\ell^1,\ell^2)|}}{n^2} - \sum_{\ell^3, \ell^4} \frac{2^{1-|P(\ell^1,\ell^2, \ell^3,\ell^4)|} \cdot F_2(a) }{n^4} - \sum_{\ell^5:\width(\ell^5) = \tau} \frac{2^{1-|P(\ell^1,\ell^2, \ell^5)|} }{n^2}
\end{aligned}
\]
Now, sum over all $\tau$-bounded pairs. We can use some fairly standard combinatorial techniques to bound these terms. In particular, we choose $t = \frac{1}{2}\log n - c$ for a large constant $c$. Then we have:

bound 1;

bound 2;

bound 3.

